Workload Equity in Vehicle Routing: The Impact of Alternative Workload Resources

In practical vehicle routing problems (VRPs), important non-monetary benefits can be achieved with more balanced operational plans which explicitly consider workload equity. This has motivated practitioners to include a wide variety of balancing criteria in decision support systems, and researchers to examine the properties of these criteria and the trade-offs made when optimizing them. As a result, previous studies have provided a much-needed understanding of how different equity functions affect the resulting VRP solutions. However, by focusing exclusively on models which balance tour lengths, a critical aspect has thus far remained unexplored -- namely the impact of the workload resource subject to the balancing. In this work, we generalize previous studies to different workload resources, extend the scope of those analyses to additional aspects of managerial and methodological significance, and reevaluate accordingly previous conclusions and guidelines for formulating a balance criterion. We propose a classification of workload resources and equity functions, and establish which general types of balanced VRP models can lead to unintended optimization outcomes. To explore in greater detail the differences between models satisfying the given guidelines, we conduct an extensive numerical study of 18 alternative balance criteria. We base our observations not only on smaller instances solved to optimality, but also on larger instances solved heuristically, to gauge the extent to which our conclusions hold also for larger VRPs. Overall, our study counter-balances the focus of previous works and reveals the importance of selecting the right workload resource.

==> sections/2-litreview.tex <==
\section{Related Literature}
\label{2-litreview}

A recent review by \cite{karsu2015} reveals that considerations of equity and balance have been gaining increased attention in various problem domains within the operations research literature. This also includes the field of logistics in particular. In fact, the relevance of equity and balance concerns in real-life VRPs is reflected by a relatively large number of application-oriented articles in a wide range of areas, including:

%\input{tables/applications}

\begin{itemize}
	\item service technician routing \citep{blakeley2003, eben2016},
	\item public utilities \citep{lin2006, groer2009, mendoza2009},
	\item vendor-managed inventory systems \citep{jang2006, day2009},
	\item waste collection \citep{kim2006, gulczynski2011, ramos2014},
	\item distribution to retail stores \citep{liu2006, kritikos2010, keskinturk2011},
	\item provision of public services such as school buses \citep{li2002} and libraries \citep{apte2006, rienthong2011}, and
	\item volunteer organizations \citep{goodson2014}.
\end{itemize}

%VRPs with balancing aspects can be found in a wide range of areas, including: service technician routing \citep{blakeley2003, eben2016}, public utilities \citep{lin2006, groer2009, mendoza2009}, vendor-managed inventory systems \citep{jang2006, day2009}, waste collection \citep{kim2006, gulczynski2011, ramos2014}, distribution to retail stores \citep{liu2006, kritikos2010, keskinturk2011}, as well as in the provision or management of public services such as school buses \citep{li2002}, libraries \citep{apte2006, rienthong2011}, and volunteer organizations \citep{goodson2014}.

It is worth noting that balancing objectives also appear at the tactical level. This is the case for example in multi-depot problems \citep{ramos2011} as well as in the context of service territory districting, including winter maintenance planning \citep{muyldermans2002, perrier2008}, beverage distribution \citep{rios2009}, and especially parcel delivery \citep{novaes2000, gonzalez2011, janssens2015, zhong2007}.

Despite the heterogeneous nature of these applications, they often share similar motivations for including equity concerns in their models and methods. Most of the cited articles describe periodic operations, and from a cost-oriented perspective, balancing the workload over the planning horizon can significantly reduce or even entirely eliminate recurring peaks in activity and their associated overtime costs \citep{day2009, groer2009, gulczynski2011}. This also has the effect of improving morale among the workforce and increasing satisfaction with operational plans, which can translate to lower rates of fluctuation and better, more consistent customer service \citep{jang2006, liu2006}. Another benefit of workload balancing is that it allows a higher utilization of existing capacity without investment in additional infrastructure \citep{apte2006}. Operational plans with more evenly spread workload are less susceptible to bottlenecks and can thus more effectively absorb variations in daily activity. This enables more robust fixed tours \citep{apte2006}, easier handling of seasonal/periodic effects \citep{day2009, eben2016}, and a flexible reaction to unexpected increases in activity \citep{blakeley2003}. Finally, in the case of public services or volunteer organizations, the issue of fairness is often just as important as cost.

Abstracting from the particularities of specific applications, many authors have proposed solution methods for more standardized problem variants. The most widely studied of these is arguably the VRP with Route Balancing (VRPRB) \citep{jozefowiez2002}, which extends the classical Capacitated VRP (CVRP) with a second objective aimed at minimizing the range of tour distances. A variety of methods have been proposed, including genetic algorithms \citep{jozefowiez2006, jozefowiez2007, jozefowiez2009}, ant colony approaches \citep{pasia2007a, pasia2007b}, greedy randomized adaptive search procedures (GRASP) \citep{oyola2014}, and decoder-based path-relinking \citep{lacomme2015}. Other authors have considered bi-objective capacitated arc routing problems \citep{lacomme2006, mei2011} and generalizations thereof \citep{mandal2015}, proposing genetic approaches, memetic algorithms, and Pareto local search as potential solution methods.

Given the number and variety of articles describing real-life VRPs with balancing aspects and those proposing \textit{methods} for their solution, it is perhaps surprising that only a handful of studies have been published that analyze more thoroughly the \textit{models} that are being solved. In the context of humanitarian relief efforts, \cite{campbell2008} and \cite{huang2012} consider the trade-offs made between total tour length and various makespan objectives aimed at balancing delivery times of aid. \cite{bertazzi2015} examine the differences between VRP solutions minimizing total tour length, and those minimizing the maximum tour length. The former articles present worst-case analyses and/or comparisons between solutions optimizing one of the potential objectives. Two more recent studies by \cite{halvorsen2016} and \cite{matl2017a} further extend these works with analyses of the Pareto-optimal compromise solutions that are obtained when using different equity functions in bi-objective VRP settings.

A common conclusion of all of these studies is that the choice of the equity objective or constraint has a significant impact on the structure of the resulting solutions, and should therefore be well-justified. However, a common limitation is that these studies have thus far considered only workload balancing in terms of tour distance. Yet the reported applications include many examples in which other resources such as the customer demand or the number of stops per tour are more relevant determinants of the workload to be balanced. To the best of our knowledge, the impact of using an alternative workload resource has thus far been unexplored, and the effect of different equity functions to measure balance has been considered only for length-based models.

In the next section we classify the various resources and functions proposed in the literature, and present some analytical properties relevant for formulating an equity objective. We report additional observations from an in-depth numerical study in Section \ref{4-results}.


==> tables/applications.tex <==
\begin{table}[]
\centering
\begin{tabular}{cc}
\textbf{Application Area}                         & \textbf{Sample References} \\ \hline
\multirow{3}{*}{waste collection}                 & \cite{kim2006}                          \\
                                                  & \cite{gulczynski2011}                          \\
                                                  & \cite{ramos2014}                          \\ \hline
\multirow{3}{*}{distribution to retail stores}    & \cite{liu2006}                          \\
                                                  & \cite{kritikos2010}                          \\
                                                  & \cite{keskinturk2011}                          \\ \hline
\multirow{3}{*}{public utilities}                 & \cite{lin2006}                          \\
                                                  & \cite{groer2009}                          \\
                                                  & \cite{mendoza2009}                          \\ \hline
\multirow{2}{*}{service technician routing}       & \cite{blakeley2003}                          \\
                                                  & \cite{eben2016}                          \\ \hline
\multirow{2}{*}{vendor-managed inventory systems} & \cite{jang2006}                          \\
                                                  & \cite{day2009}                          \\ \hline
\multirow{2}{*}{public library operations}        & \cite{apte2006}                          \\
                                                  & \cite{rienthong2011}                          \\ \hline
school bus routing                                & \cite{li2002}                          \\ \hline
volunteer organizations                           & \cite{goodson2014}                         
\end{tabular}
\caption{My caption}
\label{my-label}
\end{table}
